DVM: Towards Controllable LLM Agents in Social Deduction Games

Large Language Models (LLMs) have advanced the capability of game agents in social deduction games (SDGs). These games rely heavily on conversation-driven interactions and require agents to infer, make decisions, and express based on such information. While this progress leads to more sophisticated and strategic non-player characters (NPCs) in SDGs, there exists a need to control the proficiency of these agents. This control not only ensures that NPCs can adapt to varying difficulty levels during gameplay, but also provides insights into the safety and fairness of LLM agents. In this paper, we present DVM, a novel framework for developing controllable LLM agents for SDGs, and demonstrate its implementation on one of the most popular SDGs, Werewolf. DVM comprises three main components: Predictor, Decider, and Discussor. By integrating reinforcement learning with a win rate-constrained decision chain reward mechanism, we enable agents to dynamically adjust their gameplay proficiency to achieve specified win rates. Experiments show that DVM not only outperforms existing methods in the Werewolf game, but also successfully modulates its performance levels to meet predefined win rate targets. These results pave the way for LLM agents' adaptive and balanced gameplay in SDGs, opening new avenues for research in controllable game agents.

==> sections/relate_works.tex <==
\section{Related Works}

In recent years, LLM agents have achieved considerable success. Through reflection, tool usage, planning, and multi-agent cooperation, LLM agents have been able to realize many complex capabilities, enhancing the practical applications of LLMs\cite{shinn2024reflexion, gong2023mindagent, shen2024hugginggpt}. Some recent work has incorporated LLMs to improve agent performance in social deduction games, demonstrating their potential in understanding and generating natural language. \cite{xu2023language} proposed a framework that integrates LLMs with reinforcement learning to develop strategic language agents for the Werewolf game, outperforming existing LLM-based agents. \cite{wu2024enhance} introduced the Thinker module to enhance the reasoning capabilities of LLM-based agents in complex deduction tasks. \cite{lipinski2022emergent} and \cite{xu2023exploring} explored emergent communication strategies and tuning-free frameworks for LLMs in social deduction games. These advancements underscore the growing integration of LLMs in enhancing AI agents' performance in social deduction games. The evaluation of LLMs in playing strategic social deduction games like Avalon has been explored in \cite{light2023from}, \cite{wang2023avalon} and \cite{stepputtis-etal-2023-long}, highlighting their potential and limitations in long-horizon dialogues and deception detection. Multimodal approaches have also been investigated, as seen in \cite{lai-etal-2023-werewolf, werewolfxl}, which combined visual signals with dialogue context to model persuasion behaviors. 

Despite these advancements, existing LLM-based agents aim to maximize performance without considering controllability to player skill levels. In contrast, our approach introduces a novel framework for controllable social deduction game LLM agents that can dynamically adjust their gameplay proficiency. 
% \section{Related Works}
% \textbf{Social Deduction Game Agent in Pre-LLM Era.} In recent years, social deduction games have garnered significant attention within the AI research community. Studies have explored various aspects of deception, cooperation, and strategic play in these games. For instance, \cite{niculae-etal-2015-linguistic} examined linguistic cues that indicate betrayal in an online strategy game, revealing that subtle conversational patterns can predict impending treachery. \cite{girlea2016psycholinguistic} focused on identifying deceptive agents in the game Werewolf using psycho-linguistic features. The development of AI agents capable of reasoning and decision-making in social deduction settings has also advanced, as seen in \cite{serrino2019finding}, where a role identification algorithm was introduced to enhance agent performance in a social deduction game called The Resistance. 

% \textbf{LLM based Social Deduction Game Agent.} In recent years, LLM agents have achieved considerable success. Through reflection, tool usage, planning, and multi-agent cooperation, LLM agents have been able to realize many complex capabilities, enhancing the practical applications of LLMs\cite{shinn2024reflexion, gong2023mindagent, shen2024hugginggpt}. Some recent work has incorporated LLMs to improve agent performance in social deduction games, demonstrating their potential in understanding and generating natural language. \cite{xu2023language} proposed a framework that integrates LLMs with reinforcement learning to develop strategic language agents for the Werewolf game, outperforming existing LLM-based agents. \cite{wu2024enhance} introduced the Thinker module to enhance the reasoning capabilities of LLM-based agents in complex deduction tasks. \cite{lipinski2022emergent} and \cite{xu2023exploring} explored emergent communication strategies and tuning-free frameworks for LLMs in social deduction games. These advancements underscore the growing integration of LLMs in enhancing AI agents' performance in social deduction games. The evaluation of LLMs in playing strategic social deduction games like Avalon has been explored in \cite{light2023from}, \cite{wang2023avalon} and \cite{stepputtis-etal-2023-long}, highlighting their potential and limitations in long-horizon dialogues and deception detection. Multimodal approaches have also been investigated, as seen in \cite{lai-etal-2023-werewolf, werewolfxl}, which combined visual signals with dialogue context to model persuasion behaviors. 

% Despite these advancements, existing LLM-based agents aim to maximize performance without considering controllability to player skill levels. In contrast, our approach introduces a novel framework for controllable social deduction game LLM agents that can dynamically adjust their gameplay proficiency. 
